Neuro-Symbolic Data Generation for Math Reasoning

A critical question about Large Language Models (LLMs) is whether their apparent deficiency in mathematical reasoning is inherent, or merely a result of insufficient exposure to high-quality mathematical data. To explore this, we developed an automated method for generating high-quality, supervised mathematical datasets. The method carefully mutates existing math problems, ensuring both diversity and validity of the newly generated problems. This is achieved by a neuro-symbolic data generation framework combining the intuitive informalization strengths of LLMs, and the precise symbolic reasoning of math solvers along with projected Markov chain Monte Carlo sampling in the highly-irregular symbolic space. Empirical experiments demonstrate the high quality of data generated by the proposed method, and that the LLMs, specifically LLaMA-2 and Mistral, when realigned with the generated data, surpass their state-of-the-art counterparts.

==> tables/LLaMA-efficacy.tex <==
%We compare our model with current open-source SFT LLMs, including MetaMath~\cite{yu2023metamath}, MAmmoTH~\cite{yue23mammoth}. The original evaluation protocol of MAmmoTH combines CoT and PoT results which is not comparable with other models.
% \begin{table}[!t]
% \setlength{\columnsep}{14pt}
\begin{wraptable}{R}{0.5\linewidth}
    \centering
    \caption{Performance comparison among proprietary models, open-source general models, as well as mathematical reasoning models fine-tuned on the LLaMA-2 base model. The best performance is in bold. 
We also report delta performance between our model and other SOTA LLMs on each dataset, for various model scales.}
    \label{tab:LLaMA-performance}
    \resizebox{1\linewidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{lrrrr}
    \toprule 
    Model & \#Params & \multicolumn{1}{l|}{\#Dataset} & GSM8k & MATH \\ 
    \midrule \midrule \multicolumn{5}{c}{Proprietary Models} \\ \midrule
     GPT-4         & -    & \multicolumn{1}{l|}{-} & 92.0 & 42.5 \\
     GPT-3.5-Turbo & -    & \multicolumn{1}{l|}{-} & 80.8 & 34.1 \\
     PaLM          & 540B & \multicolumn{1}{l|}{-} & 56.5 & 8.8 \\
     PaLM-2        & 540B & \multicolumn{1}{l|}{-} & 80.7 & 34.3 \\
     Flan-PaLM-2   & 540B & \multicolumn{1}{l|}{-} & 84.7 & 33.2 \\
     Minerva       & 540B & \multicolumn{1}{l|}{-} & 58.8 & 33.6 \\
     \midrule \midrule \multicolumn{5}{c}{Open-source Models (1-10B)} \\ \midrule
     LLaMA-1       & 7B    & \multicolumn{1}{l|}{-} & 11.0 & 2.9 \\
     LLaMA-2       & 7B    & \multicolumn{1}{l|}{-} & 14.6 & 2.5 \\
     MPT           & 7B    & \multicolumn{1}{l|}{-} & 6.8 & 3.0 \\
     Falcon        & 7B    & \multicolumn{1}{l|}{-} & 6.8  & 2.3 \\
     ChatGLM-2     & 6B    & \multicolumn{1}{l|}{-} & 32.4 & - \\
     Baichuan-2    & 7B    & \multicolumn{1}{l|}{-} & 24.5 & 5.6 \\
     Mistral       & 7B    & \multicolumn{1}{l|}{-} & 52.2 & 13.1 \\
     % RFT           & 7B    & \multicolumn{1}{l|}{-} & 50.3 & - \\
     WizardMath    & 7B    & \multicolumn{1}{l|}{\raisebox{0.4ex}{\tiny $>$}96K} & 54.9 & 10.7 \\
     MuggleMATH    & 7B    & \multicolumn{1}{l|}{157K} & 68.4 & 8.4 \\
     MAmmoTH$^\dagger$       & 7B    & \multicolumn{1}{l|}{260K} & 50.5 & 10.4 \\ % From MetaMath
     % MAmmoTH$^*$       & 7B    & \multicolumn{1}{l|}{260K} & 48.7 & 8.9 \\
     % MAmmoTH$^*{\dagger}$ & 7B    & \multicolumn{1}{l|}{260K} & 22.1 & 7.6 \\
     % MAmmoTH    & 7B    & \multicolumn{1}{l|}{260K} & 53.6 & 31.5 \\ % PoT + CoT
     % MAmmoTH$^{\dagger}$ & 7B    & \multicolumn{1}{l|}{260K} & 59.4 & 33.4 \\ % PoT + CoT
     MetaMath      & 7B    & \multicolumn{1}{l|}{395K} & 66.5 & 19.8 \\ 
     \midrule
     Ours          & 7B    & \multicolumn{1}{l|}{620K}  & \textbf{76.2} & \textbf{27.1} \\ 
     \rowcolor[gray]{.9} \multicolumn{3}{c|}{$\Delta$}  
        & \textcolor{red}{$\uparrow 7.8$} 
        & \textcolor{red}{$\uparrow 7.3$} \\
     \midrule \midrule \multicolumn{5}{c}{Open-source Models (10-50B)} \\ \midrule
     LLaMA-1       & 13B    & \multicolumn{1}{l|}{-} & 17.8 & 3.9 \\
     LLaMA-1       & 34B    & \multicolumn{1}{l|}{-} & 35.6 & 7.1 \\
     LLaMA-2       & 13B    & \multicolumn{1}{l|}{-} & 28.7 & 3.9 \\
     Code-Llama    & 34B    & \multicolumn{1}{l|}{-} & 42.2 & 6.2 \\
     MPT           & 30B    & \multicolumn{1}{l|}{-} & 15.2 & 3.1 \\
     Falcon        & 40B    & \multicolumn{1}{l|}{-} & 19.6 & 2.5 \\
     Baichuan-2    & 13B    & \multicolumn{1}{l|}{-} & 52.8 & 10.1 \\
     % RFT           & 13B    & \multicolumn{1}{l|}{-} & 54.8 & -    \\
     WizardMath    & 13B    & \multicolumn{1}{l|}{\raisebox{0.4ex}{\tiny $>$}96K} & 63.9 & 14.0 \\
     MuggleMATH    & 13B    & \multicolumn{1}{l|}{157K} & 74.0 & 9.4 \\
     % MAmmoTH$^*$    & 13B    & \multicolumn{1}{l|}{260K} & 55.7 & 12.2 \\
     MAmmoTH$^\dagger$    & 13B    & \multicolumn{1}{l|}{260K} & 56.3 & 12.9 \\ % From MetaMath
     % MAmmoTH$^{*\dagger}$ & 13B    & \multicolumn{1}{l|}{260K} & 30.8 & 9.0 \\
     MAmmoTH$^{*\dagger}$ & 34B    & \multicolumn{1}{l|}{260K} & 32.6 & 11.6 \\
     % MAmmoTH$^$    & 13B    & \multicolumn{1}{l|}{260K} & 62.0 & 34.2 \\ % PoT + CoT
     % MAmmoTH$^{\dagger}$ & 13B    & \multicolumn{1}{l|}{260K} & 64.7 & 36.3 \\ % PoT + CoT
     % MAmmoTH$^{\dagger}$ & 34B    & \multicolumn{1}{l|}{260K} & 72.7 & 43.6 \\ % PoT + CoT
     MetaMath      & 13B    & \multicolumn{1}{l|}{395K} & 72.3 & 22.4 \\
     \midrule
     Ours          & 13B    & \multicolumn{1}{l|}{620K}  & \textbf{80.1} & \textbf{29.8}   \\
     \rowcolor[gray]{.9} \multicolumn{3}{c|}{$\Delta$}  
        & \textcolor{red}{$\uparrow 6.1$} 
        & \textcolor{red}{$\uparrow 7.4$} \\
     \midrule \midrule  \multicolumn{5}{c}{Open-source Models (50-70B)} \\ \midrule
     LLaMA-1       & 65B    & \multicolumn{1}{l|}{-}    & 50.9 & 10.6 \\
     LLaMA-2       & 70B    & \multicolumn{1}{l|}{-}    & 56.8 & 13.5 \\
     % RFT           & 70B    & \multicolumn{1}{l|}{-}    & 64.8 & -    \\
     % Platypus      & 70B    & \multicolumn{1}{l|}{-}    & 70.6 & 15.6 \\
     WizardMath    & 70B    & \multicolumn{1}{l|}{\raisebox{0.4ex}{\tiny $>$}96K}    & 81.6 & 22.7 \\
     MuggleMATH    & 70B    & \multicolumn{1}{l|}{157K} & 82.3 & -     \\
     MAmmoTH$^\dagger$   & 70B    & \multicolumn{1}{l|}{260K} & 72.4 & 21.1  \\ % From MetaMath
     % MAmmoTH   & 70B    & \multicolumn{1}{l|}{260K} & 76.9 & 41.8  \\ % PoT + CoT
     MetaMath      & 70B    & \multicolumn{1}{l|}{395K} & 82.3 & 26.6 \\
     \midrule
     Ours$^{\ddagger}$         & 70B    & \multicolumn{1}{l|}{620K}  & \textbf{83.8} & \textbf{27.3} \\
     \rowcolor[gray]{.9} \multicolumn{3}{c|}{$\Delta$}  
        & \textcolor{red}{$\uparrow 1.5$} 
        & \textcolor{red}{$\uparrow 0.7$} \\
    \bottomrule
    \end{tabular}
    \begin{tablenotes}
	\item[$*$] Model is fine-tuned on Code-LLaMA instead of LLaMA-2. 
        \item[$\dagger$] Model performance is re-evaluated using Pass@1 of CoT prompt. 
       \item[$\ddagger$]  Model is fine-tuned using QLoRA due to the resource limitation.
    \end{tablenotes}
    \end{threeparttable}
    }
% \end{table}
\end{wraptable}

==> tables/Mistral-efficacy.tex <==
\begin{table}[t]
    \centering
    \caption{Performance comparison among Mistral and SFT LLMs fine-tuned on Mistral. The best performance is in bold. }
    \label{tab:mistral-performance}
    % \resizebox{\linewidth}{!}{
    \begin{threeparttable}
        \begin{tabular}{lccrr}
        \toprule
        Model &\#Params & \multicolumn{1}{c|}{\#Dataset} & GSM8k & MATH   \\ 
        \midrule \midrule
        Mistral       & 7B & \multicolumn{1}{c|}{-}     & 52.2 & 13.1     \\
        % WizardMath    & 7B & \multicolumn{1}{c|}{-}   & 83.2 & 33.0     \\
        MAmmoTH$^*$   & 7B & \multicolumn{1}{c|}{260K}  & 61.9 & 17.5     \\ 
        MetaMath      & 7B & \multicolumn{1}{c|}{395K}  & 77.7 & 28.2     \\
        % MAmmoTH       & 7B & \multicolumn{1}{l|}{260K} & 75.0 & 40.0    \\ 
        \midrule
        Ours   & 7B & \multicolumn{1}{c|}{620K}  & \textbf{83.2} & \textbf{33.3} \\
        \rowcolor[gray]{.9} \multicolumn{3}{c|}{$\Delta$}  
        & \textcolor{red}{$\uparrow 5.5$} 
        & \textcolor{red}{$\uparrow 5.1$} \\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}
       \item[$*$]Model performance is re-evaluated using Pass@1 of CoT prompt. 
    \end{tablenotes}
    \end{threeparttable}
    % }
\end{table}
